Machine Learning and the Future of Bayesian Computation

Bayesian models are a powerful tool for studying complex data, allowing the analyst to encode rich hierarchical dependencies and leverage prior information. Most importantly, they facilitate a complete characterization of uncertainty through the posterior distribution. Practical posterior computation is commonly performed via MCMC, which can be computationally infeasible for high dimensional models with many observations. In this article we discuss the potential to improve posterior computation using ideas from machine learning. Concrete future directions are explored in vignettes on normalizing flows, Bayesian coresets, distributed Bayesian inference, and variational inference.

==> _preamble.tex <==
\usepackage{amsfonts,amsmath,amssymb,amsthm,mathtools,bbm,bm}
\usepackage{physics,commath,relsize}
\usepackage{graphicx,caption,subcaption,hyperref,enumitem,multirow} %authblk,
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage[nameinlink,capitalize,noabbrev]{cleveref}
\usepackage{crossreftools}
\usepackage[authoryear]{natbib}
\usepackage[title,toc]{appendix}
\usepackage[stickstoo,vvarbb]{newtxmath} %\usepackage{palatino} % times, stickstootext, fourier
\usepackage[dvipsnames,x11names]{xcolor}
\usepackage{tikz}
\usepackage{multibib} 
\newcites{S}{References}
\hypersetup{colorlinks=True, urlcolor=Blue, citecolor=MidnightBlue, linkcolor=RedViolet}

\numberwithin{equation}{section}
\newenvironment{equations}{\equation\aligned}{\endaligned\endequation}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newcommand{\assumnum}[1]{\textsf{\Alph{#1}}}
\renewcommand{\theassumption}{\assumnum{assumption}}
%\newenvironment{assumption*}[1]{\renewcommand\theassumption{#1}\assumption}{\endassumption}
\newtheorem{examplex}{Example}
\newenvironment{example}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{}\examplex}%$\clubsuit$
  {\popQED\endexamplex}
\newtheorem{remarkx}{Remark}
\newenvironment{remark}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{}\remarkx}%$\Diamond$
  {\popQED\endremarkx}

% cleverref
\crefname{assumption}{Assumption}{Assumptions}
\crefname{examplex}{Example}{Examples}
\crefname{theorem}{Theorem}{Theorems}
\crefname{section}{Section}{Sections}
\crefname{enumi}{Assumption}{Assumptions}
\crefname{equation}{Inequality}{Inequalities}
\Crefname{equation}{Equation}{Equations}
%\newcommand{\crefrangeconjunction}{--}
\pdfstringdefDisableCommands{%
    \let\Cref\crtCref
    \let\cref\crtcref
}

\def\lizhen{\textcolor{red}}
\def\ilsang{\textcolor{blue}}
%\newcommand{\newstuff}[1]{{\color{Blue}#1}}
\newcommand{\newstuff}[1]{{\color{black}#1}}
\def\vQ{\textit{Q}}
\def\hvQ{\widehat{\textit{Q}}}
\def\net{\textup{\textsf{net}}}
\def\icubes{\mathlarger{\mathlarger{\boxplus}}}
\def\mid{\mathrm{mid}}
\def\relu{\mathrm{ReLU}}
\def\SS{\texttt{\textup{SS}}}

\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}%roman numeral
\makeatother

\newcommand{\floor}[1]{\left\lfloor {#1} \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\Norm}[1]{\left\| {#1} \right\|}
\newcommand{\nnorm}[2][0]{\norm[{#1}]{{#2}}_{n,2}}
\newcommand{\fnorm}[2][0]{\norm[{#1}]{{#2}}_{\textup{F}}}
\newcommand{\opnorm}[2][0]{\norm[{#1}]{{#2}}_{\textup{op}}}
\newcommand{\inn}[2]{\left\langle {#1}, {#2} \right\rangle}

\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\def\iidsim{\stackrel{\textup{iid}}{\sim}}
\def\indsim{\stackrel{\textup{ind}}{\sim}}
\def\zero{\mathbf 0}
\def\one{\mathbf 1}
\def\ind{\mathbbm{1}}
\def\kl{\textup{KL}}
\def\supp{\textup{supp}}
\def\rank{\textup{rank}}
\def\diag{\textup{diag}}
\def\proj{\textup{Proj}}

\def\Ber{\texttt{\textup{Bernoulli}}}
\def\EXP{\texttt{\textup{Exp}}}
\def\BINOM{\texttt{\textup{Binom}}}
\def\Cat{\texttt{\textup{Cat}}}
\def\GAMMA{\texttt{\textup{Gamma}}}
\def\BETA{\texttt{\textup{Beta}}}
\def\GIG{\texttt{\textup{GIG}}}
\def\IG{\texttt{\textup{IG}}}
\def\Unif{\texttt{\textup{Unif}}}
\def\Pois{\texttt{\textup{Poisson}}}
\def\Lap{\texttt{\textup{Laplace}}}
\def\Dir{\texttt{\textup{Dirichlet}}}
\def\Geo{\texttt{\textup{Geometric}}}
\def\DP{\texttt{\textup{DP}}}
\def\N{\texttt{\textup{N}}}

\def\d{\textup{d}}
\def\e{\textup{e}}
\def\E{\mathsf{E}}
\def\P{\mathsf{P}}
\def\R{\mathbb{R}}

\makeatletter
\def\greekvectors#1{%
 \@for\next:=#1\do{%
    \def\X##1;{\expandafter\def\csname b##1\endcsname{\bm{\csname##1\endcsname}}}
    \expandafter\X\next;}
 \@for\next:=#1\do{%
    \def\X##1;{\expandafter\def\csname h##1\endcsname{\widehat{\csname##1\endcsname}}}
    \expandafter\X\next;}
 \@for\next:=#1\do{%
    \def\X##1;{\expandafter\def\csname t##1\endcsname{\widetilde{\csname##1\endcsname}}}
    \expandafter\X\next;}
 \@for\next:=#1\do{%
    \def\X##1;{\expandafter\def\csname ba##1\endcsname{\bar{\csname##1\endcsname}}}
    \expandafter\X\next;}
 \@for\next:=#1\do{%
    \def\X##1;{\expandafter\def\csname c##1\endcsname{\check{\csname##1\endcsname}}}
    \expandafter\X\next;}
 \@for\next:=#1\do{%
    \def\X##1;{\expandafter\def\csname u##1\endcsname{\underline{\csname##1\endcsname}}}
    \expandafter\X\next;}
 \@for\next:=#1\do{%
    \def\X##1;{\expandafter\def\csname hb##1\endcsname{\widehat{\bm{\csname##1\endcsname}}}}
    \expandafter\X\next;}
}
\greekvectors{alpha,beta,gamma,delta,epsilon,zeta,theta,kappa,lambda,mu,nu,xi,pi,rho,tau,sigma,phi,chi,psi,omega,varepsilon,varpi,varphi,vartheta,  Delta,Gamma,Theta,Lambda,Xi,Pi,Sigma,Phi,Psi,Omega}
    
\@tfor\next:=abfghijlmnopqrstuwxyzABCDGHIJKLMOQSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname #1\endcsname{\mathbf{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abcdeghijklnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname b#1\endcsname{\mathbbm{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abcdeghijklnpqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname t#1\endcsname{\texttt{\textup{#1}}} }
    \expandafter\command@factory\next
}
\@tfor\next:=ABCDEFGHIJKLMNOPQRSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname c#1\endcsname{\mathcal{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abdefghijklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname s#1\endcsname{\mathsf{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abcdefghjklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{
    \def\command@factory#1{\expandafter\def\csname f#1\endcsname{\mathfrak{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abcdefghjklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{
    \def\command@factory#1{\expandafter\def\csname sc#1\endcsname{\mathscr{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abcdeghijklmnopqstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname ba#1\endcsname{\bar{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=xyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname h#1\endcsname{\widehat{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abcdefghijklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{%
    \def\command@factory#1{\expandafter\def\csname ti#1\endcsname{\widetilde{#1}} }
    \expandafter\command@factory\next
}
\@tfor\next:=abcdefghjklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\do{
    \def\command@factory#1{\expandafter\def\csname u#1\endcsname{\underline{#1}} }
    \expandafter\command@factory\next
}

